Cross-Domain Video Anomaly Detection without Target Domain Adaptation

Most cross-domain unsupervised Video Anomaly Detection (VAD) works assume that at least few task-relevant target domain training data are available for adaptation from the source to the target domain. However, this requires laborious model-tuning by the end-user who may prefer to have a system that works ``out-of-the-box." To address such practical scenarios, we identify a novel target domain (inference-time) VAD task where no target domain training data are available. To this end, we propose a new `Zero-shot Cross-domain Video Anomaly Detection (zxvad)' framework that includes a future-frame prediction generative model setup. Different from prior future-frame prediction models, our model uses a novel Normalcy Classifier module to learn the features of normal event videos by learning how such features are different ``relatively" to features in pseudo-abnormal examples. A novel Untrained Convolutional Neural Network based Anomaly Synthesis module crafts these pseudo-abnormal examples by adding foreign objects in normal video frames with no extra training cost. With our novel relative normalcy feature learning strategy, zxvad generalizes and learns to distinguish between normal and abnormal frames in a new target domain without adaptation during inference. Through evaluations on common datasets, we show that zxvad outperforms the state-of-the-art (SOTA), regardless of whether task-relevant (i.e., VAD) source training data are available or not. Lastly, zxvad also beats the SOTA methods in inference-time efficiency metrics including the model size, total parameters, GPU energy consumption, and GMACs.

==> figures/error_maps.tex <==
\begin{figure}[t]
    \raggedright
    \includegraphics[width=\columnwidth]{images/error_maps.png}
    \caption{\textbf{Difference maps for abnormal frames.} We show examples of cross-domain frame prediction comparison on three datasets (source: SHT). The lighter colors in difference map mean larger prediction error indicating anomalies. Red boxes indicate ground truth anomalies. Best viewed in color.}
    \label{fig:error_maps}
  \begin{minipage}[c]{\columnwidth}
    \begin{subfigure}[t]{0.5\columnwidth}
        \raggedleft
        \input{plots/time_series_ped1}
    \end{subfigure}%
    \begin{subfigure}[t]{0.5\columnwidth}
        \raggedleft
        \input{plots/time_series_ped2}
    \end{subfigure}%
    \caption{\textbf{Anomaly detection curve.} We compare our cross-domain (source: SHT) anomaly detection on Ped1/Ped2 against \mpn. Larger value in curves indicates possible anomalies.}
    \label{fig:time_series}
  \end{minipage}
\end{figure}

==> figures/supp_amount_of_TI_data.tex <==
\begin{wrapfigure}{r}{7.8cm}
    \vspace*{-1\baselineskip}
    \centering
    \begin{subfigure}[t]{0.245\textwidth}
        \raggedright
        \input{plots/amount_hmdb}
        \caption{HMDB}
        \label{fig:amount_hmdb}
    \end{subfigure}%
    ~
    \begin{subfigure}[t]{0.245\textwidth}
        \raggedright
        \input{plots/amount_ucf101}
        \caption{UCF101}
        \label{fig:amount_ucf101}
    \end{subfigure}%
    \caption[Impact of amount of TI data on \zvad.]{\textbf{Impact of amount of TI data on} \zvad. }
    \label{fig:supp_amount_of_TI_data}
\end{wrapfigure}

==> figures/time_series.tex <==
\begin{figure}[t!]
    \vspace{-0.5em}
    \begin{subfigure}[t]{0.445\columnwidth}
        \raggedright
        \input{plots/time_series_ped1}
    \end{subfigure}%
    ~
    \hspace*{0.75em}
    \begin{subfigure}[t]{0.445\columnwidth}
        \raggedright
        \input{plots/time_series_ped2}
    \end{subfigure}%
    \vspace{-2em}
    \caption{\textbf{Anomaly detection curve.} We compare our cross-domain (source: SHT) anomaly detection on Ped1/Ped2 against \mpn. Larger value in curves indicates possible anomalies.}
    \label{fig:time_series}
    \vspace*{-1\baselineskip}
\end{figure}

==> tables/SHT_cross_domain.tex <==

\begin{table}[t]
\resizebox{\columnwidth}{!}{%
\begin{tabular}{lcccc}
\toprule
 &  & \multicolumn{3}{c}{\textbf{Testing Dataset}} \\
 \cmidrule(l){3-5} 
\multirow{-2}{*}{\textbf{Training Dataset}} & \multirow{-2}{*}{\textbf{Method}} & \textbf{Ped1} & \textbf{Ped2} & \textbf{Avenue} \\
\midrule
SH-Tech & \rgan & 73.10 & 81.95 & 71.43  \\
SH-Tech & \mpn & 74.45 & 90.17 & 74.06  \\
\rowcolor{red!10}
SH-Tech$_\text{(SH-Tech)}$ & \zvado  & \textbf{76.14} & 95.78 &  82.28 \\
\rowcolor{red!10}
SH-Tech$_\text{(HMDB51)}$ & \zvado & 75.62 & 95.74 & \textbf{83.19} \\
\rowcolor{red!10}
SH-Tech$_\text{(UCF101)}$ & \zvado & 75.41 & \textbf{95.80} & 82.25 \\
\rowcolor{red!10}
SH-Tech$_\text{(Jester)}$ & \zvado & 75.93 & 95.62 & 82.49 \\
\bottomrule
\end{tabular}%
}
\caption{\textbf{Cross-Domain Testing Comparison with SH-Tech dataset.} }
\end{table}

==> tables/TIR_cross_domain.tex <==

\begin{table}[t]
\resizebox{\columnwidth}{!}{%
\begin{tabular}{lcccc}
\toprule
 &  & \multicolumn{3}{c}{\textbf{Testing Dataset}} \\
 \cmidrule(l){3-5} 
\multirow{-2}{*}{\textbf{Training Dataset}} & \multirow{-2}{*}{\textbf{Method}} & \textbf{Ped1} & \textbf{Ped2} & \textbf{Avenue} \\
\midrule
SH-Tech & \rgan &  &  &  \\
SH-Tech & \mpn &  &  &  \\
\rowcolor{red!10}
HMDB51 & \zvado &  &  &  \\
\rowcolor{red!10}
UCF101 & \zvado &  &  &  \\
\rowcolor{red!10}
Jester & \zvado &  &  & \\
\bottomrule
\end{tabular}%
}
\caption{\textbf{Cross-Domain Testing Comparison with TIR datasets.}}
\label{tab:TIR_cross_domain}
\end{table}

==> tables/UCFCrime_cross_domain.tex <==
\begin{table}[t]
\resizebox{\columnwidth}{!}{%
\begin{tabular}{lcccc}
\toprule
 &  & \multicolumn{3}{c}{\textbf{Testing Dataset}} \\
 \cmidrule(l){3-5} 
\multirow{-2}{*}{\textbf{Training Dataset}} & \multirow{-2}{*}{\textbf{Method}} & \textbf{Ped1} & \textbf{Ped2} & \textbf{Avenue} \\
\midrule
UCF-Crime & \rgan &  66.87 & 62.53 &  64.32 \\
UCF-Crime & \mpn &  75.52 & 86.04 &  82.26 \\
\rowcolor{red!10}
UCF-Crime$_\text{(UCF-Crime)}$ & \zvado &  &  &  \\
\rowcolor{red!10}
UCF-Crime$_\text{(HMDB51)}$ & \zvado &  &  &  \\
\rowcolor{red!10}
UCF-Crime$_\text{(UCF101)}$ & \zvado &  &  &  \\
\rowcolor{red!10}
UCF-Crime$_\text{(Jester)}$ & \zvado &  &  & \\
\bottomrule
\end{tabular}%
}
\caption{\textbf{Cross-Domain Testing Comparison with UCF-Crime dataset.}}
\end{table}

==> tables/model_comparison.tex <==
\begin{table}[t]
\raggedright
\begin{minipage}[t]{0.35\columnwidth}
\resizebox{\columnwidth}{!}{%
\begin{tabular}{ccccc}
\toprule
\textbf{Method} & \begin{tabular}[c]{@{}c@{}}\textbf{Parameters}  ($\down$)\\ (millions)\end{tabular} &\textbf{GMACs} ($\down$) & \begin{tabular}[c]{@{}c@{}}\textbf{Energy} ($\down$)\\ (Joules)$^\star$\end{tabular} & \begin{tabular}[c]{@{}c@{}}\textbf{Disk Storage} ($\down$)\\ (MegaByte)\end{tabular} \\ \midrule
\rgan (paper) & 19.0 & 1384.52 & --$^\dagger$ & 79.85 \\
\mpn (code) & 12.7 & 55.09 & 10.65 & 53.14 \\
\rowcolor{red!10}
\zvado & \textbf{8.73} & \textbf{43.10} & \textbf{6.81} & \textbf{34.92} \\ \bottomrule
\end{tabular}}
\end{minipage}%
\begin{minipage}[t]{0.65\columnwidth}
\vspace{-2em}
\caption{\textbf{Comparison in the efficiency metrics.} $^\star$: we measure the GPU energy consumption by evaluating on the Ped2 dataset. $^\dagger$: \rgan does not provide its official testing code for inference-time metric evaluation.}
\vspace*{-\baselineskip}
\label{tab:efficiency}
\end{minipage}
\end{table}

==> tables/supp_background_subtraction_methods.tex <==

\begin{table}[t]
\resizebox{0.415\columnwidth}{!}{%
\begin{tabular}{cccccc}
\toprule
& &  & \multicolumn{3}{c}{\textbf{VAD Testing Data}} \\
 \cmidrule(l){4-6} 
\multirow{-2}{*}{\textbf{VAD Training Data}} &\multirow{-2}{*}{\textbf{TI Data}} &\multirow{-2}{*}{\textbf{Method}} &\textbf{Ped1} &\textbf{Ped2} &\textbf{Ave} \\
\midrule
SHT &N/A & NLAPnet \cite{roy2021predicting} (paper) & 71.60 & \textbf{95.90} & 74.70  \\
SHT &N/A & OC-AE \cite{ionescu2019object} (paper) & 74.40 & 90.30 & 78.80  \\
SHT &N/A & BA-AE \cite{georgescu2020background} (paper) & -- & 95.70 & 81.00  \\
\rowcolor{red!10}
SHT &N/A &\zvado  &\textbf{76.14} &{95.78} &82.28 \\
\rowcolor{red!10}
SHT &HMDB &\zvado &75.62 &95.74 &\textbf{83.19} \\
\rowcolor{red!10}
SHT &UCF101 &\zvado &75.41 &\underline{95.80} &82.25 \\
\rowcolor{red!10}
SHT &Jester &\zvado &\underline{75.93} &95.62 &\underline{82.49} \\
\bottomrule
\end{tabular}%
}
\caption[Comparison with background-subtraction based xVAD methods.]{\textbf{Comparison with background-subtraction based xVAD methods.} Source is SHT}
\label{tab:bg_method_exp}
\end{table}

==> tables/ti_cross_domain.tex <==
\begin{table}[t]
\centering
\raggedright
\captionsetup{width=0.985\columnwidth}
\caption{\textbf{Cross-dataset testing.} Cross-domain performance when model only trained with TI datasets. 
}
%\vspace*{-0.5em}
\resizebox{0.975\columnwidth}{!}{%
\begin{tabular}{cccccc}
\toprule
& &  & \multicolumn{3}{c}{\textbf{VAD Testing Data}} \\
 \cmidrule(l){4-6} 
\multirow{-2}{*}{\dual{\textbf{VAD Training Data}/(\textbf{Input to $\mathcal{G}(\cdot)$})}} &\multirow{-2}{*}{\dual{\textbf{Auxiliary Data}/(\textbf{Input to $\modO$})}} &\multirow{-2}{*}{\textbf{Method}} &\textbf{Ped1} &\textbf{Ped2} &\textbf{Ave} \\
\midrule
HMDB &HMDB &\zvado &\underline{76.66} & \textbf{91.53} &\textbf{81.92} \\
UCF101 &UCF101 &\zvado & {75.67} & {85.84} & \underline{81.78} \\
Jester &Jester &\zvado & \textbf{78.12} &\underline{91.23} & {78.06} \\
\bottomrule
\end{tabular}%
}
\end{table}

